Encoding Musical Style with Transformer Autoencoders

We consider the problem of learning high-level controls over the global structure of generated sequences, particularly in the context of symbolic music generation with complex language models. In this work, we present the Transformer autoencoder, which aggregates encodings of the input data across time to obtain a global representation of style from a given performance. We show it is possible to combine this global representation with other temporally distributed embeddings, enabling improved control over the separate aspects of performance style and melody. Empirically, we demonstrate the effectiveness of our method on various music generation tasks on the MAESTRO dataset and a YouTube dataset with 10,000+ hours of piano performances, where we achieve improvements in terms of log-likelihood and mean listening scores as compared to baselines.

==> old/kernel_metric.tex <==
\section{Kernel Evaluation Metric}
\label{metric}
% As a first step in devising a quantitative metric for evaluating similarities between input and output performances, we draw inspiration from \citep{jitkrittum2019kernel}. Specifically, we represent each performance as a feature vector derived from characteristic traits about the performance. Then, we compare the similarities of these feature vectors in an infinite-dimensional kernel space.
Although a variety of different metrics have been proposed to quantify both the quality \citep{engel2019gansynth} and similarity of musical performances relative to another \citep{yang2018evaluation,hung2019improving}, we note that the development of a proper metric to measure such characteristics in music generation is an open question. We build upon the ideas of \citep{hung2019improving,jitkrittum2019kernel} to capture the stylistic features of a given performance.

\subsection{Performance Features}
First, we construct a representational feature of each performance by aggregating summary statistics derived from the performance encoding: note density, average pitch, average velocity, average duration, variation of pitch, variation of velocity, and variation of duration.The note density refers to the average number of notes per second in a given performance: a higher note density often indicates a fast-moving piece, while a lower note density correlates with softer, slower pieces. The pitch denotes whether the performance is played in a higher or lower octave, velocity denotes how hard a key is pressed, and the duration describes for how long each note is pressed in a performance.

% \textbf{TODO: add table where each of these gets its own description}

\subsection{Evaluation Metric}
To compare the similarities of our constructed feature vectors, we use the Inverse Multiquadric (IMQ) kernel to project the features into an infinite-dimensional space \citep{tolstikhin2017wasserstein,jitkrittum2019kernel}:
$$k(x,y) = \frac{1}{\sqrt{||x-y||^2 + C^2}}$$
where $C$ is a tunable hyperparameter. We found empirically that the value of $C$ did not have a large effect, and set $C=10$ for our experiments. 

We project all input and generated performances into the same feature space using the IMQ kernel, and use a Maximum Mean Discrepancy (MMD)-like approach to compute the similarity between two performances. Specifically, given a single input performance $x$ and a set of conditionally-generated samples $\mathcal{Y} = \{y_i\}_{i=1}^n$:
$$-\frac{1}{n}\mathbb{E}_{x \sim p(x), y \sim q(y)}[k(x,y)] + \frac{1}{n^2} \mathbb{E}_{y,y' \sim q(y)}[k(y,y')]$$
Then, we pick the most similar performances out of the generated outputs according to this metric. We omit the usual first term in the MMD loss that quantifies the similarity between the input sets when we only have one conditioning input performance. In the case that we have a one-to-one mapping between an input performance and an output sample $x \rightarrow y$, we work with the kernel similarity directly: $k(x,y)$. We demonstrate empirically that this kernel metric identifies the relevant characteristics of interest in our generated performances in Section~\ref{experiments}.

% There are a few other metrics proposed to quantify the quality and similarity of musical performances, as noted in \citep{yang2018evaluation,hung2019improving}. However, we note that \kristy{TODO}.

==> old/old_experiments.tex <==
% \section{Experiments}
% \label{experiments}
% \paragraph{Datasets} We used both MAESTRO \citep{hawthorne2018enabling} and \dataset datasets \citep{simon2019} for the experimental setup. We used the standard 80/10/10 train/validation/test split from MAESTRO v1.0.0, and augmented the dataset by 10x using pitch shifts of no more than a minor third and time stretches of at most 5\%. We note that this augmentation is distinct from the noise-injection procedure referenced in Section~\ref{c_generation}: the data augmentation merely increases the size of the initial dataset, while the perturbation procedure operates \textit{only} on the input performance signal. The \dataset dataset did not require any additional augmentation.

% \paragraph{Experimental Setup} We implemented the model in the Tensor2Tensor framework \citep{vaswani2017attention}, and used the default hyperparameters for training: 0.2 learning rate with 8000 warmup steps, \texttt{rsqrt\_decay}, 0.2 dropout, and early stopping for GPU training. For TPU training, we use AdaFactor with the \texttt{rsqrt\_decay} and learning rate warmup steps to be 10K. We adopt many of the hyperparameter configurations from \citep{huang2018music}, where we reduce the query and key hidden size to half the hidden size, use 8 hidden layers, use 384 hidden units, and set the maximum relative distance to consider to half the training sequence length for relative global attention. We set the maximum sequence length to be 2048 tokens, and a filter size of 1024. We provide additional details on the model architectures and hyperparameter configurations in Appendix C.

% \subsection{Log-Likelihood Evaluation}
% As expected, we find that the Transformer autoencoder framework with the encoder output bottleneck outperforms other baselines. In Tables~\ref{table:perf_nll} and 2, we see that all conditional model variants outperform their unconditional counterparts. Interestingly, we find that for the melody \& performance model, different methods of combining the embeddings work better for different datasets. For example, \texttt{concatenate} led to the lowest NLL for the \dataset dataset, while \texttt{sum} outperformed all other variants for MAESTRO. We report NLL values for both MAESTRO and the \dataset dataset for the perturbed-input model variants in Appendix B.

% \begin{table}[h]
% \centering 
% \begin{tabular}{l|l|l}
% \toprule
% \textbf{Model variation} & MAESTRO & \dataset \\
% \midrule
% Unconditional model with rel. attention \citep{huang2018music} & 1.840 & 1.49 \\ 
% \midrule
% Performance autoencoder with rel. attention (ours) & \textbf{1.799} & \textbf{1.384}\\   
% \bottomrule
% \end{tabular}
% \caption{Note-wise test NLL on the MAESTRO and \dataset datasets, with event-based representations of lengths $L = 2048$. We exclude the performance autoencoder baseline (no aggregation) as it memorized the data ($\text{NLL}=0$). Conditional models outperformed their unconditional counterparts.}
% \label{table:perf_nll}
% \end{table}

% \begin{table}[h]
% \centering
% \begin{tabular}{l|l|l}
% \toprule
% \textbf{Model variation} & MAESTRO & \dataset \\
% \midrule
% Melody-only Transformer with rel. attention \citep{huang2018music} & 1.786 & 1.302\\ 
% \midrule
% Melody \& performance autoencoder with rel. attention, sum (ours) & \textbf{1.706} & 1.275\\   
% Melody \& performance autoencoder with rel. attention, concat (ours) & 1.713 & \textbf{1.237}\\   
% Melody \& performance autoencoder with rel. attention, tile (ours) & 1.709 & 1.248\\ 
% \bottomrule
% \end{tabular}
% \caption{Note-wise test NLL on the MAESTRO and \dataset datasets with melody conditioning, with event-based representations of lengths $L = 2048$. We note that \texttt{sum} worked best for MAESTRO, while \texttt{concatenate} outperformed all other baselines for the \dataset dataset.}
% \label{table:melody_nll}
% \end{table}

% \subsection{Similarity Evaluation}
% We use our similarity metric to evaluate whether using a conditioning signal in both the (a) performance autoencoder and (b) melody \& performance autoencoder produces samples that are more similar in style to the conditioning inputs from the evaluation set relative to other baselines.

% First, we sample 500 examples from the evaluation set and use them as conditioning signals to generate one sample for each input. Then, we compare each conditioning signal to: (1) the generated sample and (2) an unconditional sample. We compute the similarity metric as defined in Section~\ref{metric} pairwise and take the average over 500 examples. As shown in Table 3, we find that the performance autoencoder generates samples that have 36\% higher similarity to the conditioning input as compared to the unconditional baseline.

% \begin{table}[h]
% \centering
% \begin{tabular}{l|l|l}
% \toprule
% \textbf{Similarity Metric} & MAESTRO & \dataset \\
% \midrule
% Performance autoencoder (ours) & \textbf{0.0840} & \textbf{0.0944}\\ 
% Unconditional baseline \citep{huang2018music} & 0.0455 & 0.0694 \\
% \midrule
% Melody \& performance autoencoder (ours) & 0.147 & 0.157 \\
% Melody-only Transformer \citep{huang2018music} & 0.110 & 0.145 \\
% Performance-only autoencoder (ours) & \textbf{0.172} & \textbf{0.161} \\
% Unconditional baseline \citep{huang2018music} & 0.005 & 0.138 \\
% \bottomrule
% \end{tabular}
% \caption{Average similarities for both the performance and melody \& performance autoencoders.}
% \label{table:similiarity_metric}
% \end{table}

% For the melody \& performance autoencoder, we sample 717*2 distinct performances -- we reserve one set of 717 for conditioning performance styles, and the other set of 717 we use to extract melodies in order to synthesize in the style of a \textit{different} performance. We compare the melody \& performance autoencoder to 3 different baselines: (1) one that is conditioned only on the melody (Melody-only); (2) conditioned only on performance (Performance-only); and (3) an unconditional language model. Interestingly, we find that the kernel evaluation metric is more sensitive to the performance style than melodic similarity. Table 3 demonstrates that the Melody-only autoencoder suffers without the performance conditioning, while the Performance-only model performs best. The Melody \& performance autoencoder performs comparably to the best model.
% % Table 3 shows that although Performance-only shares the most similarities to the conditioning input, the melody \& performance autoencoder produces samples that are comparable, while the unconditional baseline is the least similar out of all.

% \subsection{Interpolations}
% \subsubsection{Performance Autoencoder}
% In this experiment, we test whether the performance autoencoder can successfully interpolate between different performances. First, we sample 1000 performances from the \dataset test set (100 for MAESTRO, due to its smaller size), and split this dataset in half. The first half we reserve for the original starting performance, which we call ``performance A", and the other half we reserve for the end performance, denoted as ``performance B." Then we use the performance encoder to encode performance A into its compressed representation $z_A$, and do the same for performance B to obtain $z_B$. For a range $\alpha \in [0, 0.125, \ldots, 0.875, 1.0]$, we sample a new performance $\text{perf}_{\text{new}}$ that results from decoding $\alpha \cdot z_A + (1 - \alpha) \cdot z_B$. We observe how the similarity metric defined in Section~\ref{metric} changes between this newly interpolated performance $\text{perf}_{\text{new}}$ and performances \{A, B\}.

% % (which we denote $x$) and interpolated sample y to obtain IMQ(x, y) for all 500 performances. Then, we compute the same IMQ(x, y) for all 500 performances in the set of performance B with the newly interpolated samples.
% % Specifically, we compute the $\KL_{\text{avg}}(x||y)$ between each input performance A (which we denote $x$) and interpolated sample $y$ for all 500 performances. Then, we compute the same $\KL_{\text{avg}}(x||y)$ for all 500 performances $x$ in the set of performance B with the newly interpolated samples $y$. 

% \begin{figure}[h]
% \centering
% \includegraphics[width=.6\textwidth]{figures/yt_perf_interp.pdf}
% \caption{For the \dataset dataset, the relative distance from performance A ($\alpha=1$) to the interpolated sample increases as $\alpha$ is slowly increased to 1.0.}
% \label{fig:interp_dist}
% \end{figure}

% Specifically, we compute the kernel similarity using the IMQ kernel between each input performance A and interpolated sample $\text{perf}_{\text{new}}$  for all 500 samples, and compute the same pairwise similarity for each performance B. We then compute the normalized distance between each interpolated sample and the corresponding performance A or B, which we denote as: $\texttt{rel\_distance(perf A)} = 1 - \frac{\texttt{sim\_A}}{\texttt{sim\_A + sim\_B}}$, where $\texttt{sim\_A}$ is defined by our kernel similarity metric. We average this distance across all elements in the set and find in Figure~\ref{fig:interp_dist} that the relative distance between performance A slowly increases as we increase $\alpha$ from 0 to 1, as expected. We note that it is not possible to conduct this interpolation study with non-aggregated baselines, as we cannot interpolate across variable-length embeddings. We find that a similar trend holds for MAESTRO as in Figure 3(a).

% \begin{figure}[h]
% \centering
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=.9\textwidth]{figures/yt_mel_interp.pdf}
% \caption{Relative distance to performance A}
% \end{subfigure}
% ~
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=.9\textwidth]{figures/yt_mel_interp_between_mel.pdf}
% \caption{Relative distance to melody A}
% \end{subfigure}
% \caption{For the \dataset dataset, relative distance from performance A ($\alpha=1$) as $\alpha$ is slowly increased to 1.0 while the conditioned melody remains fixed. As in (b), we note that the relative distance to the fixed conditioning melody with respect to a random performance remains fixed while the interpolation is conducted between performances A and B, which shows that we can control for elements of style and melody separately.}
% \label{fig:interp_dist_mel}
% \end{figure}

% \subsubsection{Melody \& Performance Autoencoder}
% We conduct a similar study as above, now with the melody \& performance autoencoder. For this study, we hold out 716 unique melody-performance pairs (where the melody is not derived from the same performance) from the \dataset evaluation dataset and 50 examples from MAESTRO. We then interpolate across the different performances, while keeping the conditioning melody input the same across the interpolations.

% As shown in Figure 3(a), we find that a similar trend holds as in the performance autoencoder: the newly-interpolated samples show that the relative distance between performance A increases as we increase the corresponding value of $\alpha$. We note that the interpolation effect is slightly lower than that of the previous section, particularly because the interpolated sample is also dependent on the melody that it is conditioned on. Interestingly, in Figure 3(b), we note that the relative distance between the input performance from which we derived the original melody remains fairly constant across the interpolation procedure. This suggests that we are able to factorize out the two sources of variation and that varying the axis of the input performance keeps the variation in melody constant.


% \subsection{Human Evaluation}
% We also conducted listening studies to evaluate the perceived effect of performance and melody conditioning on the generated output. Using models trained on the \dataset dataset, we conducted two studies: one for performance conditioning, and one for melody and performance conditioning.

% \begin{figure}[h]
% \centering
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=.8\textwidth]{figures/performance.pdf}
% % \caption{}
% \end{subfigure}
% ~
% \begin{subfigure}[b]{0.49\textwidth}
% \includegraphics[width=.9\textwidth]{figures/performance_and_melody.pdf}
% % \caption{}
% \end{subfigure}
% \caption{Results of our listening studies, showing the number of times each source won in a pairwise comparison. Black error bars indicate estimated standard deviation of means.}
% \label{fig:listening_tests}
% \end{figure}

% % \subsubsection{Performance Conditioning}
% For performance conditioning, we presented participants with a 20s performance clip from the evaluation dataset that we used as a conditioning signal. We then asked them to listen to two additional 20s performance clips and use a Likert scale to rate which one sounded most similar in style to the conditioning signal. The sources the participants rated included ``Ground Truth" (a different snippet of the same sample used for the conditioning signal), ``Conditioned" (output of the Performance Autoencoder), and ``Unconditioned" (output of unconditional model). For this study, 492 ratings were collected, with each source involved in 328 pair-wise comparisons.

% % \subsubsection{Melody and Performance Conditioning}
% For melody and performance conditioning, we presented participants with a 20s performance clip from the evaluation dataset and a 20s melody from a different piece in the evaluation dataset that we used as our conditioning signals. We then asked them to listen to two additional 20s performance clips and use a Likert scale to rate which sounded most like the conditioning melody played in the style of the conditioning performance. The sources the participants rated included ``Melody \& Performance" (output of the Melody-Performance Autoencoder), ``Melody only" (output of a model conditioned only on the melody signal), ``Performance only" (output of a model conditioned only on the performance signal), and ``Unconditioned" (output of an unconditional model). For this study, 714 ratings were collected, with each source involved in 357 pair-wise comparisons.

% \Figref{fig:listening_tests} shows the number of comparisons in which each source was selected as being most similar in style to the conditioning signal. A Kruskal-Wallis H test of the ratings showed that there is at least one statistically significant difference between the models: $\chi^2(2) = 332.09,~p < 0.05~(7.72\mathrm{e}{-73})$ for melody conditioning and $\chi^2(2) = 277.74,~p < 0.05~(6.53\mathrm{e}{-60})$ for melody and performance conditioning. A post-hoc analysis using the Wilcoxon signed-rank test with Bonferroni correction showed that there were statistically significant differences between all pairs of the performance study with $p < 0.05/3$ and all pairs of the performance and melody study with $p < 0.05/6$ except between the ``Melody only" and ``Melody \& Performance" models ($p = 0.0894$).

% These results demonstrate that the performance conditioning signal has a clear effect on the generated output. In fact, the effect was sufficiently robust that in the 164 comparisons between ``Ground Truth" and ``Conditioned", participants said they had a preference for ``Conditioned" 58 times.

% Even though the results between ``Melody-only" and ``Melody \& Performance" are close, this study demonstrates that conditioning with both melody and performance results in outputs that are better at achieving the goal than conditioning on performance alone, and they are competitive with melody-only conditioning, despite the model having to deal with the complexity of incorporating both conditioning signals. In fact, we find quantitative evidence that human evaluation is more sensitive to melodic similarity, as the ``Performance-only" model performs worst -- a stark contrast to the results from the kernel evaluation metric in Section 5.2.

% We provide several audio examples demonstrating the effectiveness of these conditioning signals in the online supplement at \exampleswebpage. Our qualitative findings from the audio examples and interpolations, coupled with the quantitative results from the similarity metric and the listening test which capture different aspects of the synthesized performance, support the finding that the Melody \& Performance autoencoder offers significant control over the generated samples.


% % \begin{table}[h]
% % \centering
% % \begin{tabular}{l|l|l}
% % \toprule
% % \textbf{Similarity Metric} & MAESTRO & \dataset \\
% % \midrule
% % Performance autoencoder (ours) & \textbf{0.48} & \textbf{0.72}\\ 
% % Unconditional baseline \citep{huang2018music} & 0.0455 & 3.84 \\
% % \midrule
% % Melody + performance autoencoder (ours) & 0.147 & 0.157 \\
% % Melody-only Transformer \citep{huang2018music} & 0.110 & 0.145 \\
% % Performance-only autoencoder (ours) & \textbf{0.172} & \textbf{0.161} \\
% % Unconditional baseline \citep{huang2018music} & 0.005 & 0.138 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Average similarity metric note-wise for both the performance and melody+performance autoencoders for lengths $L = 2048$.}
% % \label{table:similiarity_metric}
% % \end{table}

% % \begin{table}[h]
% % \centering
% % \begin{tabular}{l|l|l}
% % \toprule
% % \textbf{similarity Metric} & MAESTRO & \dataset \\
% % \midrule
% % Performance autoencoder (ours) & \textbf{0.48} & \textbf{0.72}\\ 
% % Unconditional baseline \citep{huang2018music} & 9.69 & 3.84 \\
% % \midrule
% % Melody + performance autoencoder (ours) & \textbf{2.33} & \textbf{17.33} \\
% % Melody-only Transformer \citep{huang2018music} & 3.91 & 20.56 \\
% % Performance-only autoencoder (ours) & 3.29 & 29.62\\
% % Unconditional baseline \citep{huang2018music} & 20.22 & 22.99 \\
% % \bottomrule
% % \end{tabular}
% % \caption{Average distance between samples for both the performance and melody+performance autoencoders for the MAESTRO and \dataset datasets. Lower is better.}
% % \label{table:similarity_metric}
% % \end{table}

==> old/old_metric.tex <==
\section{Similarity Evaluation Metric}
\label{metric}
Although a variety of different metrics have been proposed to quantify both the quality \citep{engel2019gansynth} and similarity of musical performances relative to another \citep{yang2018evaluation,hung2019improving}, we note that the development of a proper metric to measure such characteristics in music generation is an open question. 
As a first step towards quantifying similarity, we build upon the ideas of \citep{hung2019improving} to capture the stylistic features of a given performance.

\subsection{Performance Features}
First, we construct a distributional representation of each performance by utilizing two key statistics derived from its event-based encoding: note density and pitch \citep{yang2018evaluation}. The note density refers to the average number of notes per second in a given performance: a higher note density often indicates a fast-moving piece, while a lower note density correlates with softer, slower pieces. The pitch denotes whether the performance is played in a higher or lower octave. 

% After experimenting with simple descriptive statistics of the entire performance such as average pitch and velocity, we found that such features were insufficient to describe the underlying comple
To best capture the salient features within the periodic structure of a musical performance, we used a sliding window of 2s to construct two histograms of the average note density and pitch within each window. We then fit a Gaussian distribution to each histogram, and represent each performance in terms of the mean $\mu$ and variance $\sigma^2$ of these two Gaussians.

\subsection{Evaluation Metric}
To quantify how different two performances are, we use the Kullback-Leibler (KL) divergence between each performance's (1) note density and (2) pitch distributions. Specifically, for both note density and pitch, we compute:
$$\KL(p||q) = \log \frac{\sigma_2}{\sigma_1} + \frac{\sigma_1^2 + (\mu_1 - \mu_2)^2}{2\sigma_2^2} - \frac{1}{2}$$
where $p \sim \mathcal{N}(\mu_1, \sigma_1)$ and $q \sim \mathcal{N}(\mu_2, \sigma_2)$ are univariate Gaussians.

To "symmetrize" the KL, we then compute: 
$$\KL_{\text{pitch}} = \frac{1}{2}\KL(p||q) + \frac{1}{2}\KL(q||p)$$
$$\KL_{\text{density}} = \frac{1}{2}\KL(p||q) + \frac{1}{2}\KL(q||p)$$
and define the final distance metric as:
$$\KL_{\text{avg}} = \frac{1}{2}\left(\KL_{\text{pitch}} + \KL_{\text{density}} \right)$$

We use the metric $\KL_{\text{avg}}$ to quantify how different two musical performances are in terms of their relative note density and pitch, and demonstrate empirically that this metric identifies the relevant characteristics of interest in our generated performances in Section~\ref{experiments}.

% \kristy{potentially revamp metric: Trying out a KL approach after fitting two Gaussians to sliding-window mean note density and mean pitch}
% As a first step in devising a quantitative metric for evaluating similarities between input and output performances, we draw inspiration from \citep{jitkrittum2019kernel}. Specifically, we represent each performance as a feature vector derived from characteristic traits about the performance. Then, we compare the similarities of these feature vectors in an infinite-dimensional kernel space.

% \subsection{Performance Features}
% First, we construct a representational feature of each performance by aggregating summary statistics derived from the performance encoding: note density, average pitch, average velocity, average duration, variation of pitch, variation of velocity, and variation of duration. The note density refers to the average number of notes per second in a given performance: a higher note density will frequently indicate a fast-moving piece, while a lower note density correlates with slower pieces. The pitch denotes the pitch of the keys (whether the performance is played in a higher or lower octave), and the duration describes how long on average each note is pressed in a performance.

% % \textbf{TODO: add table where each of these gets its own description}

% \subsection{Evaluation Metric}
% We note that a wide variety of kernels exist for comparison. We use the Inverse Multiquadric (IMQ) kernel to compare two performance feature vectors \citep{jitkrittum2019kernel,tolstikhin2017wasserstein}:
% $$k(x,y) = \frac{1}{\sqrt{||x-y||^2 + C^2}}$$
% where $C$ is a tunable hyperparameter. We found that the value of $C$ did not have a large effect, and set $C=10$ for our experiments. 

% We projected all input and generated performances into the same infinite-dimensional space using this IMQ kernel, and used a Maximum Mean Discrepancy (MMD)-like approach to compute the similarity between two performances. Specifically, given a single input performance $x$ and a set of conditionally-generated samples $\mathcal{Y} = \{y\}_{i=1}^n$:

% $$-\frac{1}{n}\mathbb{E}_{x \sim p(x), y \sim q(y)}[k(x,y)] + \frac{1}{n^2} \mathbb{E}_{y,y' \sim q(y)}[k(y,y')]$$

% Then, we pick the most similar performances out of the generated outputs according to this metric. We omit the usual first term in the MMD loss that quantifies the similarity between the input sets in the case that we only have one conditioning input performance. In the case that we have a one-to-one mapping between an input performance and an output sample, we work with the kernel similarity directly: $k(x,y)$. We demonstrate empirically that this kernel metric identifies the relevant characteristics of interest in our generated performances in Section~\ref{experiments}.

% There are a few other metrics proposed to quantify the quality and similarity of musical performances, as noted in \citep{yang2018evaluation,hung2019improving}. However, we note that \kristy{TODO}.
